Derivation of a Relation for the Steepening of TeV Selected Blazar Gamma-ray Spectra with Energy and Redshift

We derive a relation for the steepening of blazar gamma-ray spectra between the multi-GeV Fermi energy range and the TeV energy range observed by atmospheric Cerenkov telescopes. The change in spectral index is produced by two effects: (1) an intrinsic steepening, independent of redshift, owing to the properties of emission and absorption in the source, and (2) a redshift-dependent steepening produced by intergalactic pair production interactions of blazar gamma-rays with low energy photons of the intergalactic background light (IBL). Given this relation, with good enough data on the mean gamma-ray SED of TeV selected BL Lacs, the redshift evolution of the IBL can, in principle, be determined independently of stellar evolution models. We apply our relation to the results of new Fermi observations of TeV selected blazars.

==> graphicx <==
%%
%% This is file `graphicx.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% graphicx.dtx  (with options: `package')
%% 
%% graphicx.dtx Copyright (C) 1994      David Carlisle Sebastian Rahtz
%%              Copyright (C) 1995 1996 1997 1999 David Carlisle
%%
%% This file is part of the Standard LaTeX `Graphics Bundle'.
%% It may be distributed under the terms of the LaTeX Project Public
%% License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesPackage{graphicx}
          [1999/02/16 v1.0f  Enhanced LaTeX Graphics (DPC,SPQR)]
\DeclareOption{unknownkeysallowed}
  {\PassOptionsToPackage\CurrentOption{keyval}}
\DeclareOption*{\PassOptionsToPackage\CurrentOption{graphics}}
\ProcessOptions
\RequirePackage{keyval,graphics}
\define@key{Gin}{bb}
           {\Gin@bboxtrue\Gread@parse@bb#1 \\}
\define@key{Gin}{bbllx}
           {\Gin@bboxtrue\Gin@defaultbp\Gin@llx{#1}}
\define@key{Gin}{bblly}
           {\Gin@bboxtrue\Gin@defaultbp\Gin@lly{#1}}
\define@key{Gin}{bburx}
           {\Gin@bboxtrue\Gin@defaultbp\Gin@urx{#1}}
\define@key{Gin}{bbury}
           {\Gin@bboxtrue\Gin@defaultbp\Gin@ury{#1}}
\define@key{Gin}{hiresbb}[true]{%
  \edef\Gread@BBox{%
    \@percentchar\@percentchar
    \csname if#1\endcsname HiRes\fi
    BoundingBox}}
\let\KV@Gin@natwidth\KV@Gin@bburx
\let\KV@Gin@natheight\KV@Gin@bbury
\define@key{Gin}{viewport}
           {\let\Gin@viewport@code\Gin@viewport\Gread@parse@vp#1 \\}
\define@key{Gin}{trim}
           {\let\Gin@viewport@code\Gin@trim\Gread@parse@vp#1 \\}
\def\Gread@parse@vp#1 #2 #3 #4 #5\\{%
  \Gin@defaultbp\Gin@vllx{#1}%
  \Gin@defaultbp\Gin@vlly{#2}%
  \Gin@defaultbp\Gin@vurx{#3}%
  \Gin@defaultbp\Gin@vury{#4}}%
\def\Gin@viewport{%
  \let\Gin@ollx\Gin@llx
  \let\Gin@olly\Gin@lly
  \let\Gin@ourx\Gin@urx
  \let\Gin@oury\Gin@ury
  \dimen@\Gin@llx\p@\advance\dimen@ \Gin@vurx\p@
                      \edef\Gin@urx{\strip@pt\dimen@}%
  \dimen@\Gin@lly\p@\advance\dimen@ \Gin@vury\p@
                      \edef\Gin@ury{\strip@pt\dimen@}%
  \dimen@\Gin@llx\p@\advance\dimen@ \Gin@vllx\p@
                      \edef\Gin@llx{\strip@pt\dimen@}%
  \dimen@\Gin@lly\p@\advance\dimen@ \Gin@vlly\p@
                      \edef\Gin@lly{\strip@pt\dimen@}}
\def\Gin@trim{%
  \let\Gin@ollx\Gin@llx
  \let\Gin@olly\Gin@lly
  \let\Gin@ourx\Gin@urx
  \let\Gin@oury\Gin@ury
  \dimen@\Gin@llx\p@\advance\dimen@ \Gin@vllx\p@
                      \edef\Gin@llx{\strip@pt\dimen@}%
  \dimen@\Gin@lly\p@\advance\dimen@ \Gin@vlly\p@
                      \edef\Gin@lly{\strip@pt\dimen@}%
  \dimen@\Gin@urx\p@\advance\dimen@ -\Gin@vurx\p@
                      \edef\Gin@urx{\strip@pt\dimen@}%
  \dimen@\Gin@ury\p@\advance\dimen@ -\Gin@vury\p@
                      \edef\Gin@ury{\strip@pt\dimen@}}
\let\Gin@vllx\Gin@llx\let\Gin@vlly\Gin@llx
\let\Gin@vurx\Gin@llx\let\Gin@vury\Gin@llx
\define@key{Gin}{angle}
           {\Gin@esetsize
            \@tempswatrue
            \edef\@tempa{\toks@{\noexpand\Gin@erotate{#1}{\the\toks@}}}%
            \@tempa}
\define@key{Gin}{origin}[c]{%
  \def\Gin@erotate{\Grot@box@kv[origin=#1]}}
\define@key{Gin}{width}{\def\Gin@ewidth{#1}}
\define@key{Gin}{height}{\def\Gin@eheight{#1}}
\define@key{Gin}{totalheight}{%
  \def\Gin@eresize{\totalheight}\def\Gin@eheight{#1}}
\define@key{Gin}{keepaspectratio}[true]{%
  \lowercase{\Gin@boolkey{#1}}{iso}}
\define@key{Gin}{scale}{%
  \if@tempswa
    \edef\@tempa{\toks@{\noexpand\Gscale@box{#1}[#1]{\the\toks@}}}%
    \@tempa
  \else
    \def\Gin@req@sizes{%
      \def\Gin@scalex{#1}\let\Gin@scaley\Gin@exclamation
      \Gin@req@height\Gin@scalex\Gin@nat@height
      \Gin@req@width\Gin@scalex\Gin@nat@width}%
  \fi
  \@tempswatrue}
\define@key{Gin}{draft}[true]{%
  \lowercase{\Gin@boolkey{#1}}{draft}}
\define@key{Gin}{clip}[true]{%
  \lowercase{\Gin@boolkey{#1}}{clip}}
\define@key{Gin}{type}{%
  \def\Ginclude@graphics##1{%
    \begingroup
    \def\Gin@base{##1}%
    \edef\@tempa{{#1}{\Gin@eread}{\Gin@ecom{##1\Gin@eext}}}%
    \expandafter\Gin@setfile\@tempa
    \endgroup}}
\define@key{Gin}{ext}{\def\Gin@eext{#1}}
\let\Gin@eext\@empty
\define@key{Gin}{read}{%
 \def\Gin@eread{#1}%
 \def\@tempa{*}\ifx\@tempa\Gin@eread\def\Gin@eread{\Gin@eext}\fi}
\let\Gin@eread\@empty
\define@key{Gin}{command}{\def\Gin@ecom##1{#1}}
\let\Gin@ecom\@firstofone
\def\Gin@boolkey#1#2{%
  \csname Gin@#2\ifx\relax#1\relax true\else#1\fi\endcsname}
\def\Gin@eresize{\height}
\def\Gin@esetsize{%
  \let\@tempa\Gin@exclamation
  \if@tempswa
    \edef\@tempa{\toks@{\noexpand
             \Gscale@@box\noexpand\Gin@eresize
              {\Gin@ewidth}{\Gin@eheight}{\the\toks@}}}%
    \@tempa
  \else
    \ifx\Gin@ewidth\@tempa
      \ifx\Gin@eheight\@tempa
      \else
         \let\Gin@@eheight\Gin@eheight
         \def\Gin@req@sizes{%
           \Gscale@div\Gin@scaley\Gin@@eheight\Gin@nat@height
           \let\Gin@scalex\Gin@exclamation
           \setlength\Gin@req@height\Gin@@eheight
           \Gin@req@width\Gin@scaley\Gin@nat@width}%
      \fi
    \else
      \ifx\Gin@eheight\@tempa
         \let\Gin@@ewidth\Gin@ewidth
         \def\Gin@req@sizes{%
           \Gscale@div\Gin@scalex\Gin@@ewidth\Gin@nat@width
           \let\Gin@scaley\Gin@exclamation
           \setlength\Gin@req@width\Gin@@ewidth
           \Gin@req@height\Gin@scalex\Gin@nat@height}%
      \else
         \let\Gin@@ewidth\Gin@ewidth
         \let\Gin@@eheight\Gin@eheight
         \def\Gin@nosize##1{%
           \KV@Gin@natwidth\Gin@@ewidth
           \KV@Gin@natheight\Gin@@eheight}%
         \def\Gin@req@sizes{%
           \Gscale@div\Gin@scalex\Gin@@ewidth\Gin@nat@width
           \Gscale@div\Gin@scaley\Gin@@eheight\Gin@nat@height
           \ifGin@iso
             \ifdim\Gin@scaley\p@>\Gin@scalex\p@
               \let\Gin@scaley\Gin@scalex
             \else
               \let\Gin@scalex\Gin@scaley
             \fi
           \fi
           \Gin@req@width\Gin@scalex\Gin@nat@width
           \Gin@req@height\Gin@scaley\Gin@nat@height}%
       \fi
     \fi
  \fi
  \let\Gin@ewidth\Gin@exclamation
  \let\Gin@eheight\Gin@ewidth}
\newdimen\Gin@req@height
\newdimen\Gin@req@width
\let\Gin@outer@scalex\relax
\let\Gin@outer@scaley\relax
\let\Gin@angle\relax
\let\Gin@ewidth\Gin@exclamation
\let\Gin@eheight\Gin@ewidth
\def\Gin@scalex{1}
\let\Gin@scaley\Gin@exclamation
\def\Gin@i{%
 \def\Gin@req@sizes{%
   \Gin@req@height\Gin@nat@height
   \Gin@req@width\Gin@nat@width}%
 \@ifnextchar[\Gin@ii{\Gin@ii[]}}
\def\Gin@ii[#1]#2{%
    \def\@tempa{[}\def\@tempb{#2}%
    \ifx\@tempa\@tempb
      \def\@tempa{\Gin@iii[#1][}%
      \expandafter\@tempa
    \else
     \begingroup
       \@tempswafalse
       \toks@{\Ginclude@graphics{#2}}%
       \setkeys{Gin}{#1}%
       \Gin@esetsize
       \the\toks@
     \endgroup
     \fi}
\def\rotatebox{%
  \@ifnextchar[\Grot@box@kv\Grot@box@std}
\def\Grot@box@std#1#2{%
  \Grot@setangle{#1}%
  \setbox\z@\hbox{{#2}}%
  \Grot@x\z@
  \Grot@y\z@
  \Grot@box}
\def\Grot@box@kv[#1]#2#3{%
  \@begin@tempboxa\hbox{#3}%
    \Grot@x\width \divide\Grot@x\tw@
    \Grot@y\height \advance\Grot@y-\depth \divide\Grot@y\tw@
    \setkeys{Grot}{#1}%
    \setbox\z@\box\@tempboxa
    \Grot@setangle{#2}%
    \Grot@box
  \@end@tempboxa}
\define@key{Grot}{origin}[c]{%
 \@tfor\@tempa:=#1\do{%
    \if l\@tempa \Grot@x\z@\else
    \if r\@tempa \Grot@x\width\else
    \if t\@tempa \Grot@y\height\else
    \if b\@tempa \Grot@y-\depth\else
    \if B\@tempa \Grot@y\z@\fi\fi\fi\fi\fi}}
\define@key{Grot}{x}{\setlength\Grot@x{#1}}
\define@key{Grot}{y}{\setlength\Grot@y{#1}}
\define@key{Grot}{units}{%
  \def\Grot@setangle##1{%
  \dimen@##1\p@
  \dimen@ii#1\p@
  \divide\dimen@ii360\relax
  \divide\dimen@\dimen@ii
  \edef\Grot@angle{\number\dimen@}}}
\let\Gin@erotate\Grot@box@std
\endinput
%%
%% End of file `graphicx.sty'.
